ICPE: An Item Cluster-Wise Pareto-Efficient Framework for Recommendation Debiasing

Recommender system based on historical user-item interactions is of vital importance for web-based services. However, the observed data used to train the recommender model suffers from severe bias issues. Practically, the item frequency distribution of the dataset is a highly skewed power-law distribution. Interactions of a small fraction of head items account for almost the whole training data. The normal training paradigm from such biased data tends to repetitively generate recommendations from the head items, which further exacerbates the biases and affects the exploration of potentially interesting items from the niche set. In this work, we innovatively explore the central theme of recommendation debiasing from an item cluster-wise multi-objective optimization perspective. Aiming to balance the learning on various item clusters that differ in popularity during the training process, we propose a model-agnostic framework namely Item Cluster-Wise Pareto-Efficient Recommendation (ICPE). In detail, we define our item cluster-wise optimization target as the recommender model should balance all item clusters that differ in popularity, thus we set the model learning on each item cluster as a unique optimization objective. To achieve this goal, we first explore items' popularity levels from a novel causal reasoning perspective. Then, we devise popularity discrepancy-based bisecting clustering to separate the item clusters. Next, we adaptively find the overall harmonious gradient direction for cluster-wise optimization objectives from a Pareto-efficient solver. Finally, in the prediction stage, we perform counterfactual inference to further eliminate the impact of global propensity. Extensive experimental results verify the superiorities of ICPE on overall recommendation performance and biases elimination.

==> ICMRec <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{jambor2010optimizing}
T.~Jambor and J.~Wang, ``Optimizing multiple objectives in collaborative
  filtering,'' in \emph{RecSys}, 2010, pp. 55--62.

\bibitem{mcnee2006being}
S.~M. McNee, J.~Riedl, and J.~A. Konstan, ``Being accurate is not enough: how
  accuracy metrics have hurt recommender systems,'' in \emph{CHI'06}, 2006, pp.
  1097--1101.

\bibitem{ge2010beyond}
M.~Ge, C.~Delgado-Battenfeld, and D.~Jannach, ``Beyond accuracy: evaluating
  recommender systems by coverage and serendipity,'' in \emph{Proceedings of
  the fourth ACM conference on Recommender systems}, 2010, pp. 257--260.

\bibitem{rendle2012bpr}
S.~Rendle, C.~Freudenthaler, Z.~Gantner, and L.~Schmidt-Thieme, ``Bpr: Bayesian
  personalized ranking from implicit feedback,'' \emph{arXiv preprint
  arXiv:1205.2618}, 2012.

\bibitem{chen2020bias}
J.~Chen, H.~Dong, X.~Wang, F.~Feng, M.~Wang, and X.~He, ``Bias and debias in
  recommender system: A survey and future directions,'' \emph{arXiv preprint
  arXiv:2010.03240}, 2020.

\bibitem{hurley2013personalised}
N.~J. Hurley, ``Personalised ranking with diversity,'' in \emph{Proceedings of
  the 7th ACM conference on Recommender systems}, 2013, pp. 379--382.

\bibitem{kaminskas2016diversity}
M.~Kaminskas and D.~Bridge, ``Diversity, serendipity, novelty, and coverage: a
  survey and empirical analysis of beyond-accuracy objectives in recommender
  systems,'' \emph{TiiS}, vol.~7, no.~1, pp. 1--42, 2016.

\bibitem{chen2020improving}
W.~Chen, P.~Ren, F.~Cai, F.~Sun, and M.~de~Rijke, ``Improving end-to-end
  sequential recommendations with intent-aware diversification,'' in
  \emph{CIKM}, 2020, pp. 175--184.

\bibitem{ribeiro2012pareto}
M.~T. Ribeiro, A.~Lacerda, A.~Veloso, and N.~Ziviani, ``Pareto-efficient
  hybridization for multi-objective recommender systems,'' in \emph{Proceedings
  of the sixth ACM conference on Recommender systems}, 2012, pp. 19--26.

\bibitem{ribeiro2014multiobjective}
M.~T. Ribeiro, N.~Ziviani, E.~S.~D. Moura, I.~Hata, A.~Lacerda, and A.~Veloso,
  ``Multiobjective pareto-efficient approaches for recommender systems,''
  \emph{TIST}, vol.~5, no.~4, pp. 1--20, 2014.

\bibitem{musto2017multi}
C.~Musto, M.~de~Gemmis, G.~Semeraro, and P.~Lops, ``A multi-criteria
  recommender system exploiting aspect-based sentiment analysis of users'
  reviews,'' in \emph{Proceedings of the eleventh ACM conference on recommender
  systems}, 2017, pp. 321--325.

\bibitem{nguyen2017multi}
P.~Nguyen, J.~Dines, and J.~Krasnodebski, ``A multi-objective learning to
  re-rank approach to optimize online marketplaces for multiple stakeholders,''
  \emph{arXiv preprint arXiv:1708.00651}, 2017.

\bibitem{rodriguez2012multiple}
M.~Rodriguez, C.~Posse, and E.~Zhang, ``Multiple objective optimization in
  recommender systems,'' in \emph{Proceedings of the sixth ACM conference on
  Recommender systems}, 2012, pp. 11--18.

\bibitem{zitzler2001spea2}
E.~Zitzler, M.~Laumanns, and L.~Thiele, ``Spea2: Improving the strength pareto
  evolutionary algorithm,'' \emph{TIK-report}, vol. 103, 2001.

\bibitem{xiao2017fairness}
L.~Xiao, Z.~Min, Z.~Yongfeng, G.~Zhaoquan, L.~Yiqun, and M.~Shaoping,
  ``Fairness-aware group recommendation with pareto-efficiency,'' in
  \emph{Proceedings of the Eleventh ACM Conference on Recommender Systems},
  2017, pp. 107--115.

\bibitem{wang2016multi}
S.~Wang, M.~Gong, H.~Li, and J.~Yang, ``Multi-objective optimization for long
  tail recommendation,'' \emph{Knowledge-Based Systems}, vol. 104, pp.
  145--155, 2016.

\bibitem{cui2017novel}
L.~Cui, P.~Ou, X.~Fu, Z.~Wen, and N.~Lu, ``A novel multi-objective evolutionary
  algorithm for recommendation systems,'' \emph{Journal of Parallel and
  Distributed Computing}, vol. 103, pp. 53--63, 2017.

\bibitem{lin2019pareto}
X.~Lin, H.~Chen, C.~Pei, F.~Sun, X.~Xiao, H.~Sun, Y.~Zhang, W.~Ou, and
  P.~Jiang, ``A pareto-efficient algorithm for multiple objective optimization
  in e-commerce recommendation,'' in \emph{Proceedings of the 13th ACM
  Conference on Recommender Systems}, 2019, pp. 20--28.

\bibitem{desideri2009multiple}
J.-A. D{\'e}sid{\'e}ri, ``Multiple-gradient descent algorithm (mgda),'' 2009.

\bibitem{sener2018multi}
O.~Sener and V.~Koltun, ``Multi-task learning as multi-objective
  optimization,'' \emph{Advances in Neural Information Processing Systems},
  vol.~31, pp. 527--538, 2018.

\bibitem{adomavicius2011improving}
G.~Adomavicius and Y.~Kwon, ``Improving aggregate recommendation diversity
  using ranking-based techniques,'' \emph{IEEE Transactions on Knowledge and
  Data Engineering}, vol.~24, no.~5, pp. 896--911, 2011.

\bibitem{li2017two}
J.~Li, K.~Lu, Z.~Huang, and H.~T. Shen, ``Two birds one stone: on both
  cold-start and long-tail recommendation,'' in \emph{Proceedings of the 25th
  ACM international conference on Multimedia}, 2017, pp. 898--906.

\bibitem{anderson2006long}
C.~Anderson, \emph{The Long Tail}.\hskip 1em plus 0.5em minus 0.4em\relax
  Hachette Books, 2006.

\bibitem{yin2012challenging}
H.~Yin, B.~Cui, J.~Li, J.~Yao, and C.~Chen, ``Challenging the long tail
  recommendation,'' \emph{arXiv preprint arXiv:1205.6700}, 2012.

\bibitem{goel2010anatomy}
S.~Goel, A.~Broder, E.~Gabrilovich, and B.~Pang, ``Anatomy of the long tail:
  ordinary people with extraordinary tastes,'' in \emph{Proceedings of the
  third ACM international conference on Web search and data mining}, 2010, pp.
  201--210.

\bibitem{shi2013trading}
L.~Shi, ``Trading-off among accuracy, similarity, diversity, and long-tail: a
  graph-based recommendation approach,'' in \emph{Proceedings of the 7th ACM
  conference on Recommender systems}, 2013, pp. 57--64.

\bibitem{johnson2017enhancing}
J.~Johnson and Y.-K. Ng, ``Enhancing long tail item recommendations using
  tripartite graphs and markov process,'' in \emph{Proceedings of the
  International Conference on Web Intelligence}, 2017, pp. 761--768.

\bibitem{wu2019pd}
Q.~Wu, Y.~Liu, C.~Miao, B.~Zhao, Y.~Zhao, and L.~Guan, ``Pd-gan: Adversarial
  learning for personalized diversity-promoting recommendation.'' in
  \emph{IJCAI}, vol.~19, 2019, pp. 3870--3876.

\bibitem{kim2019sequential}
Y.~Kim, K.~Kim, C.~Park, and H.~Yu, ``Sequential and diverse recommendation
  with long tail.'' in \emph{IJCAI}, 2019, pp. 2740--2746.

\bibitem{bai2017dltsr}
B.~Bai, Y.~Fan, W.~Tan, and J.~Zhang, ``Dltsr: A deep learning framework for
  recommendation of long-tail web services,'' \emph{IEEE Transactions on
  Services Computing}, 2017.

\bibitem{ke2017lightgbm}
G.~Ke, ``Lightgbm: A highly efficient gradient boosting decision tree,'' in
  \emph{Advances in neural information processing systems}, 2017, pp.
  3146--3154.

\bibitem{rendle2010factorization}
S.~Rendle, ``Factorization machines,'' in \emph{2010 IEEE International
  Conference on Data Mining}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2010, pp. 995--1000.

\bibitem{zhou2010solving}
T.~Zhou, Z.~Kuscsik, J.-G. Liu, M.~Medo, J.~R. Wakeling, and Y.-C. Zhang,
  ``Solving the apparent diversity-accuracy dilemma of recommender systems,''
  \emph{PNAS}, vol. 107, no.~10, pp. 4511--4515, 2010.

\bibitem{schaffler2002stochastic}
S.~Sch{\"a}ffler, R.~Schultz, and K.~Weinzierl, ``Stochastic method for the
  solution of unconstrained vector optimization problems,'' \emph{Journal of
  Optimization Theory and Applications}, vol. 114, no.~1, pp. 209--222, 2002.

\bibitem{kendall2018multi}
A.~Kendall, Y.~Gal, and R.~Cipolla, ``Multi-task learning using uncertainty to
  weigh losses for scene geometry and semantics,'' in \emph{CVPR}, 2018, pp.
  7482--7491.

\bibitem{desideri2012multiple}
J.-A. D{\'e}sid{\'e}ri, ``Multiple-gradient descent algorithm (mgda) for
  multiobjective optimization,'' \emph{Comptes Rendus Mathematique}, vol. 350,
  no. 5-6, pp. 313--318, 2012.

\bibitem{makimoto1994efficient}
N.~Makimoto, I.~Nakagawa, and A.~Tamura, ``An efficient algorithm for finding
  the minimum norm point in the convex hull of a finite point set in the
  plane,'' \emph{OPER RES LETT}, vol.~16, no.~1, pp. 33--40, 1994.

\bibitem{koren2009matrix}
Y.~Koren, R.~Bell, and C.~Volinsky, ``Matrix factorization techniques for
  recommender systems,'' \emph{Computer}, vol.~42, no.~8, pp. 30--37, 2009.

\bibitem{jaggi2013revisiting}
M.~Jaggi, ``Revisiting frank-wolfe: Projection-free sparse convex
  optimization,'' in \emph{International Conference on Machine Learning}.\hskip
  1em plus 0.5em minus 0.4em\relax PMLR, 2013, pp. 427--435.

\bibitem{rifai2011contractive}
S.~Rifai, P.~Vincent, X.~Muller, X.~Glorot, and Y.~Bengio, ``Contractive
  auto-encoders: Explicit invariance during feature extraction,'' in
  \emph{Icml}, 2011.

\bibitem{larger2012photonic}
L.~Larger, ``Photonic information processing beyond turing: an optoelectronic
  implementation of reservoir computing,'' \emph{Optics express}, vol.~20,
  no.~3, pp. 3241--3249, 2012.

\bibitem{liang2016modeling}
D.~Liang, L.~Charlin, J.~McInerney, and D.~M. Blei, ``Modeling user exposure in
  recommendation,'' in \emph{Proceedings of the 25th international conference
  on World Wide Web}, 2016, pp. 951--961.

\bibitem{he2016ups}
R.~He and J.~McAuley, ``Ups and downs: Modeling the visual evolution of fashion
  trends with one-class collaborative filtering,'' in \emph{proceedings of the
  25th international conference on world wide web}, 2016, pp. 507--517.

\bibitem{jarvelin2002cumulated}
K.~J{\"a}rvelin and J.~Kek{\"a}l{\"a}inen, ``Cumulated gain-based evaluation of
  ir techniques,'' \emph{ACM Transactions on Information Systems (TOIS)},
  vol.~20, no.~4, pp. 422--446, 2002.

\bibitem{tang2020long}
K.~Tang, J.~Huang, and H.~Zhang, ``Long-tailed classification by keeping the
  good and removing the bad momentum causal effect,'' \emph{arXiv preprint
  arXiv:2009.12991}, 2020.

\bibitem{he2020lightgcn}
X.~He, ``Lightgcn: Simplifying and powering graph convolution network for
  recommendation,'' in \emph{SIGIR}, 2020, pp. 639--648.

\bibitem{wang2019neural}
X.~Wang, X.~He, M.~Wang, F.~Feng, and T.-S. Chua, ``Neural graph collaborative
  filtering,'' in \emph{Proceedings of the 42nd international ACM SIGIR
  conference on Research and development in Information Retrieval}, 2019, pp.
  165--174.

\bibitem{he2017neural}
X.~He, L.~Liao, H.~Zhang, L.~Nie, X.~Hu, and T.-S. Chua, ``Neural collaborative
  filtering,'' in \emph{WWW}, 2017, pp. 173--182.

\bibitem{mnih2007probabilistic}
A.~Mnih and R.~R. Salakhutdinov, ``Probabilistic matrix factorization,''
  \emph{Advances in neural information processing systems}, vol.~20, pp.
  1257--1264, 2007.

\bibitem{kingma2014adam}
D.~P. Kingma and J.~Ba, ``Adam: A method for stochastic optimization,''
  \emph{arXiv preprint arXiv:1412.6980}, 2014.

\bibitem{chen2018gradnorm}
Z.~Chen, V.~Badrinarayanan, C.-Y. Lee, and A.~Rabinovich, ``Gradnorm: Gradient
  normalization for adaptive loss balancing in deep multitask networks,'' in
  \emph{International Conference on Machine Learning}.\hskip 1em plus 0.5em
  minus 0.4em\relax PMLR, 2018, pp. 794--803.

\bibitem{kang2019decoupling}
B.~Kang, S.~Xie, M.~Rohrbach, Z.~Yan, A.~Gordo, J.~Feng, and Y.~Kalantidis,
  ``Decoupling representation and classifier for long-tailed recognition,''
  \emph{arXiv preprint arXiv:1910.09217}, 2019.

\bibitem{chen2020esam}
Z.~Chen, ``Esam: Discriminative domain adaptation with non-displayed items to
  improve long-tail performance,'' in \emph{Proceedings of the 43rd
  International ACM SIGIR Conference on Research and Development in Information
  Retrieval}, 2020, pp. 579--588.

\bibitem{wu2007karush}
H.-C. Wu, ``The karush--kuhn--tucker optimality conditions in an optimization
  problem with interval-valued objective function,'' \emph{European Journal of
  Operational Research}, vol. 176, no.~1, pp. 46--59, 2007.

\bibitem{liu2019real}
Y.~Liu, K.~Ge, X.~Zhang, and L.~Lin, ``Real-time attention based look-alike
  model for recommender system,'' in \emph{Proceedings of the 25th ACM SIGKDD
  International Conference on Knowledge Discovery \& Data Mining}, 2019, pp.
  2765--2773.

\bibitem{yu2019vaegan}
X.~Yu, X.~Zhang, Y.~Cao, and M.~Xia, ``Vaegan: A collaborative filtering
  framework based on adversarial variational autoencoders.'' in \emph{IJCAI},
  2019, pp. 4206--4212.

\bibitem{AbdollahpouriBM17}
H.~Abdollahpouri, ``Controlling popularity bias in learning-to-rank
  recommendation,'' in \emph{Proceedings of the Eleventh {ACM} Conference on
  Recommender Systems, RecSys 2017, Como, Italy, August 27-31, 2017}.

\bibitem{jannach2015recommenders}
D.~Jannach, L.~Lerche, I.~Kamehkhosh, and M.~Jugovac, ``What recommenders
  recommend: an analysis of recommendation biases and possible
  countermeasures,'' \emph{UMUI}, vol.~25, no.~5, pp. 427--491, 2015.

\bibitem{KrishnanSSS18}
A.~Krishnan and A.~Sharma, ``An adversarial approach to improve long-tail
  performance in neural collaborative filtering,'' in \emph{Proceedings of the
  27th {ACM} International Conference on Information and Knowledge Management,
  {CIKM} 2018, Torino, Italy, October 22-26, 2018}, A.~Cuzzocrea, Ed.\hskip 1em
  plus 0.5em minus 0.4em\relax {ACM}, 2018, pp. 1491--1494.

\bibitem{reynolds2009gaussian}
D.~A. Reynolds, ``Gaussian mixture models.'' \emph{Encyclopedia of biometrics},
  vol. 741, pp. 659--663, 2009.

\bibitem{gruson2019offline}
A.~Gruson, P.~Chandar, C.~Charbuillet, J.~McInerney, S.~Hansen, and D.~Tardieu,
  ``Offline evaluation to make decisions about playlistrecommendation
  algorithms,'' in \emph{WSDM}, 2019, pp. 420--428.

\bibitem{abdollahpouri2017controlling}
H.~Abdollahpouri, R.~Burke, and B.~Mobasher, ``Controlling popularity bias in
  learning-to-rank recommendation,'' in \emph{Proceedings of the Eleventh ACM
  Conference on Recommender Systems}, 2017, pp. 42--46.

\bibitem{likas2003global}
A.~Likas, N.~Vlassis, and J.~J. Verbeek, ``The global k-means clustering
  algorithm,'' \emph{Pattern recognition}, vol.~36, no.~2, pp. 451--461, 2003.

\bibitem{jang2020cities}
S.~Jang, H.~Lee, H.~Cho, and S.~Chung, ``Cities: Contextual inference of
  tail-item embeddings for sequential recommendation,'' in \emph{ICDM}.\hskip
  1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 202--211.

\bibitem{zhang2021model}
Y.~Zhang, D.~Z. Cheng, T.~Yao, X.~Yi, L.~Hong, and E.~H. Chi, ``A model of two
  tales: Dual transfer learning framework for improved long-tail item
  recommendation,'' in \emph{WWW 2021}, 2021, pp. 2220--2231.

\bibitem{huang2006correcting}
J.~Huang, A.~Gretton, K.~Borgwardt, B.~Sch{\"o}lkopf, and A.~Smola,
  ``Correcting sample selection bias by unlabeled data,'' \emph{Advances in
  neural information processing systems}, vol.~19, pp. 601--608, 2006.

\bibitem{xu2018representation}
K.~Xu, C.~Li, Y.~Tian, T.~Sonobe, K.-i. Kawarabayashi, and S.~Jegelka,
  ``Representation learning on graphs with jumping knowledge networks,'' in
  \emph{International Conference on Machine Learning}.\hskip 1em plus 0.5em
  minus 0.4em\relax PMLR, 2018, pp. 5453--5462.

\bibitem{tang2020investigating}
X.~Tang, H.~Yao, Y.~Sun, Y.~Wang, J.~Tang, C.~Aggarwal, P.~Mitra, and S.~Wang,
  ``Investigating and mitigating degree-related biases in graph convoltuional
  networks,'' in \emph{Proceedings of the 29th ACM International Conference on
  Information \& Knowledge Management}, 2020, pp. 1435--1444.

\bibitem{hinton2006reducing}
G.~E. Hinton and R.~R. Salakhutdinov, ``Reducing the dimensionality of data
  with neural networks,'' \emph{science}, vol. 313, no. 5786, pp. 504--507,
  2006.

\bibitem{misztal2021bias}
J.~Misztal-Radecka and B.~Indurkhya, ``Bias-aware hierarchical clustering for
  detecting the discriminated groups of users in recommendation systems,''
  \emph{Information Processing \& Management}, vol.~58, no.~3, p. 102519, 2021.

\bibitem{swaminathan2015self}
A.~Swaminathan and T.~Joachims, ``The self-normalized estimator for
  counterfactual learning,'' \emph{advances in neural information processing
  systems}, vol.~28, 2015.

\bibitem{wan2022cross}
Q.~Wan, X.~He, X.~Wang, J.~Wu, W.~Guo, and R.~Tang, ``Cross pairwise ranking
  for unbiased item recommendation,'' in \emph{Proceedings of the ACM Web
  Conference 2022}, 2022, pp. 2370--2378.

\bibitem{scholkopf2022causality}
B.~Sch{\"o}lkopf, ``Causality for machine learning,'' in \emph{Probabilistic
  and Causal Inference: The Works of Judea Pearl}, 2022, pp. 765--804.

\bibitem{wang2017research}
X.~Wang and L.~Wang, ``Research on intrusion detection based on feature
  extraction of autoencoder and the improved k-means algorithm,'' in \emph{2017
  10th International Symposium on Computational Intelligence and Design
  (ISCID)}, vol.~2.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp.
  352--356.

\bibitem{zhang2021causal}
Y.~Zhang, F.~Feng, X.~He, T.~Wei, C.~Song, G.~Ling, and Y.~Zhang, ``Causal
  intervention for leveraging popularity bias in recommendation,'' in
  \emph{Proceedings of the 44th International ACM SIGIR Conference on Research
  and Development in Information Retrieval}, 2021, pp. 11--20.

\bibitem{lee2022bilateral}
J.-w. Lee, S.~Park, J.~Lee, and J.~Lee, ``Bilateral self-unbiased learning from
  biased implicit feedback,'' 2022.

\bibitem{saito2020unbiased}
Y.~Saito, S.~Yaginuma, Y.~Nishino, H.~Sakata, and K.~Nakata, ``Unbiased
  recommender learning from missing-not-at-random implicit feedback,'' in
  \emph{Proceedings of the 13th International Conference on Web Search and Data
  Mining}, 2020, pp. 501--509.

\bibitem{saito2020ubpr}
Y.~Saito, ``Unbiased pairwise learning from biased implicit feedback,'' in
  \emph{Proceedings of the 2020 ACM SIGIR on International Conference on Theory
  of Information Retrieval}, 2020, pp. 5--12.

\bibitem{ren2018learning}
M.~Ren, W.~Zeng, B.~Yang, and R.~Urtasun, ``Learning to reweight examples for
  robust deep learning,'' in \emph{International conference on machine
  learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2018, pp. 4334--4343.

\bibitem{chen2021autodebias}
J.~Chen, H.~Dong, Y.~Qiu, X.~He, X.~Xin, L.~Chen, G.~Lin, and K.~Yang,
  ``Autodebias: Learning to debias for recommendation,'' in \emph{Proceedings
  of the 44th International ACM SIGIR Conference on Research and Development in
  Information Retrieval}, 2021, pp. 21--30.

\bibitem{zhu2020unbiased}
Z.~Zhu, Y.~He, Y.~Zhang, and J.~Caverlee, ``Unbiased implicit recommendation
  and propensity estimation via combinational joint learning,'' in
  \emph{Fourteenth ACM Conference on Recommender Systems}, 2020, pp. 551--556.

\bibitem{wei2021model}
T.~Wei, F.~Feng, J.~Chen, Z.~Wu, J.~Yi, and X.~He, ``Model-agnostic
  counterfactual reasoning for eliminating popularity bias in recommender
  system,'' in \emph{Proceedings of the 27th ACM SIGKDD Conference on Knowledge
  Discovery \& Data Mining}, 2021, pp. 1791--1800.

\bibitem{wang2021deconfounded}
W.~Wang, F.~Feng, X.~He, X.~Wang, and T.-S. Chua, ``Deconfounded recommendation
  for alleviating bias amplification,'' in \emph{Proceedings of the 27th ACM
  SIGKDD Conference on Knowledge Discovery \& Data Mining}, 2021, pp.
  1717--1725.

\bibitem{zheng2021disentangling}
Y.~Zheng, C.~Gao, X.~Li, X.~He, Y.~Li, and D.~Jin, ``Disentangling user
  interest and conformity for recommendation with causal embedding,'' in
  \emph{Proceedings of the Web Conference 2021}, 2021, pp. 2980--2991.

\bibitem{hu2008collaborative}
Y.~Hu, Y.~Koren, and C.~Volinsky, ``Collaborative filtering for implicit
  feedback datasets,'' in \emph{2008 Eighth IEEE international conference on
  data mining}.\hskip 1em plus 0.5em minus 0.4em\relax Ieee, 2008, pp.
  263--272.

\bibitem{bonner2018causal}
S.~Bonner and F.~Vasile, ``Causal embeddings for recommendation,'' in
  \emph{Proceedings of the 12th ACM conference on recommender systems}, 2018,
  pp. 104--112.

\bibitem{liu2020general}
D.~Liu, P.~Cheng, Z.~Dong, X.~He, W.~Pan, and Z.~Ming, ``A general knowledge
  distillation framework for counterfactual recommendation via uniform data,''
  in \emph{Proceedings of the 43rd International ACM SIGIR Conference on
  Research and Development in Information Retrieval}, 2020, pp. 831--840.

\bibitem{schnabel2016recommendations}
T.~Schnabel, A.~Swaminathan, A.~Singh, N.~Chandak, and T.~Joachims,
  ``Recommendations as treatments: Debiasing learning and evaluation,'' in
  \emph{international conference on machine learning}.\hskip 1em plus 0.5em
  minus 0.4em\relax PMLR, 2016, pp. 1670--1679.

\bibitem{liu2021mitigating}
D.~Liu, P.~Cheng, H.~Zhu, Z.~Dong, X.~He, W.~Pan, and Z.~Ming, ``Mitigating
  confounding bias in recommendation via information bottleneck,'' in
  \emph{Fifteenth ACM Conference on Recommender Systems}, 2021, pp. 351--360.

\bibitem{yu2020influence}
J.~Yu, H.~Zhu, C.-Y. Chang, X.~Feng, B.~Yuan, X.~He, and Z.~Dong, ``Influence
  function for unbiased recommendation,'' in \emph{Proceedings of the 43rd
  International ACM SIGIR Conference on Research and Development in Information
  Retrieval}, 2020, pp. 1929--1932.

\end{thebibliography}

